Rethinking Normalization Methods in Federated Learning

Federated learning (FL) is a popular distributed learning framework that can reduce privacy risks by not explicitly sharing private data. In this work, we explicitly uncover external covariate shift problem in FL, which is caused by the independent local training processes on different devices. We demonstrate that external covariate shifts will lead to the obliteration of some devices' contributions to the global model. Further, we show that normalization layers are indispensable in FL since their inherited properties can alleviate the problem of obliterating some devices' contributions. However, recent works have shown that batch normalization, which is one of the standard components in many deep neural networks, will incur accuracy drop of the global model in FL. The essential reason for the failure of batch normalization in FL is poorly studied. We unveil that external covariate shift is the key reason why batch normalization is ineffective in FL. We also show that layer normalization is a better choice in FL which can mitigate the external covariate shift and improve the performance of the global model. We conduct experiments on CIFAR10 under non-IID settings. The results demonstrate that models with layer normalization converge fastest and achieve the best or comparable accuracy for three different model architectures.

==> Design.tex <==
\section{Federated Averaging with Feature Normalization}

% \subsection{Normalziation}
% \textcolor{red}{Introduce the layer normalization or group normalization and their insights on the external covariate shift formally}

% To tackle the external covariate shift in FL, we propose a new federated learning method -- FedNorm, which is based on FedAvg but can also be extended to other FL methods. Similar to FedAvg, FedNorm aggregates updated local models through weighted averaging on the central server. However, FedNorm requires the devices to conduct feature normalization during local training such that different local models will have the similar feature distributions for the same channel. In this section, We will elaborate the local feature normalization and provide a theoretical analysis to explain why our proposed feature normalization can mitigate external covariate shift.

% \subsection{Local Feature Normalization}

% %\PY{(should we use $f(\cdot,\mW)$?)}

% Considering a DNN $f(\cdot,\mW)$ that can be represented layer by layer as $f(\cdot, \mW) := [f^1(\cdot, \mW^1), f^2(\cdot, \mW^2), ..., f^L(\cdot, \mW^L)]$, our feature normalization is to normalize the features of each layer to follow specific distributions for different channels. We assume that the features of a channel follow Gaussian distribution, which is a common assumption used by BatchNorm. Then our normalization of a layer $f^l(\cdot,\mW^l)$ can be formulated as:

% \begin{equation}
%     R(\mW^l) =  \sum\limits_c|| \mu[{f^l(\vx^l, \mW^l)}_{c}] -  \mu^l_c||^2_2 + || \sigma[{f^l(\vx^l, \mW^l)}_{c}] -  \sigma^l_c||^2_2,
% \end{equation}

% where $f^l(\vx^l, \mW)_{c}$ represents the feature of the $c$-th channel in the $l$-th layer given the input $\vx^l$ to that layer. $\mu[.]$ and $\sigma[.]$ represent the mean and standard deviation, respectively. $\mu_c^l$ and $\sigma_c^l$ are the targeted mean and variance value of the feature of the $c$-th channel in the $l$-th layer that we aim to normalize to. In this work, we set $m_c^l$ and $v_c^l$ to be 0 and 1 respectively such that the features of each channel are normalized to follow normal distribution. After applying the feature normalization, the local training objective of the $k$-th client in FedNorm is defined as:

% \begin{equation}
%     F_k(W) = CE_k(W) + \alpha \sum\limits_{l\in [L]}R(W^l),
% \end{equation}
% where $CE_k(\cdot)$ is the cross entropy loss of the $k$-th client, $\alpha$ controls the strength of feature normalization.
% Note that our feature normalization for one layer is only based on the output and input of this layer, so the normalization of all layers can be done simultaneously, which is time efficient, rather than through back-propagation. During federated training, all the devices apply local feature normalization with the same $\{\mu_c^l|l\in[L]\}$ and $\{\sigma_c^l|l\in[L]\}$ during local training. 
% In doing so, the features of each channel follow the same distribution on different devices, and hence the  external covariate shift can be effectively addressed. 

\subsection{Rethinking External Covariate Shift and Feature Normalization} \label{sec:rethink}

To better understand why our proposed feature normalization can effectively mitigate the external covariate shift in FL, we describe the impact of our normalization on model parameters. For simplicity, we use the fully connected (FC) layer as an example for analysis. Note that such an analysis can be naturally extended to other types of layers. Specifically, a FC layer is represented as:

\begin{equation}
    \vy = \mW \vx + \vb,
\end{equation}

where $\vx$ is the input to this layer, $\mW$ and $\vb$ are weight and bias, $\vy$ is the feature of this layer. We assume that the input features $\vx$ for this layer are whitened (independently distributed with zero mean and unit variance), then $\mu[\vy]=\mu[\vb]$ and $\sigma[\vy]=||\mW||$ where $||.||$ denotes the Euclidean norm. For two sets of weights $\mW_1$ and $\mW_2$, if their feature deviations have significant discrepancies, i.e., $\sigma[\vy_1] \gg \sigma[\vy_2]$, then we can derive that $||\mW_1||\gg||\mW_2||$. Thus, the essence of external covariate shift describes the shift of model parameter's norm. Considering these two sets of weights belong to two local models involved in FL, then the contribution of $\mW_2$ will be obliterated by $\mW_1$ as shown in Figure~\ref{fig:rethink}, and the same effect applies to the bias, which is more related to $\mu[\vy]$.

\begin{figure*}[ht]
\centering
     \includegraphics[scale=0.35]{image/rethink.pdf}
\caption{The contribution of the model with a smaller norm will be obliterated by the model with a larger norm during aggregation.}
\label{fig:rethink}
\end{figure*}

In FL, it is reasonable that weights on different devices are diverse due to non-IID data, but they should have similar norms $||\mW||$, otherwise the aggregated model would be dominated by a small part of local models with larger wight norms. Our feature normalization forces $\mW$ on different devices to have similar norms, such that the contributions of certain devices will not be obliterated by the others.
